Integration of Polyimide Flexible PCB Wings in Northeastern Aerobat

The principal aim of this Master's thesis is to propel the optimization of the membrane wing structure of the Northeastern Aerobat through origami techniques and enhancing its capacity for secure hovering within confined spaces. Bio-inspired drones offer distinctive capabilities that pave the way for innovative applications, encompassing wildlife monitoring, precision agriculture, search and rescue operations, as well as the augmentation of residential safety. The evolved noise-reduction mechanisms of birds and insects prove advantageous for drones utilized in tasks like surveillance and wildlife observation, ensuring operation devoid of disturbances. Traditional flying drones equipped with rotary or fixed wings encounter notable constraints when navigating narrow pathways. While rotary and fixed-wing systems are conventionally harnessed for surveillance and reconnaissance, the integration of onboard sensor suites within micro aerial vehicles (MAVs) has garnered interest in vigilantly monitoring hazardous scenarios in residential settings. Notwithstanding the agility and commendable fault tolerance exhibited by systems such as quadrotors in demanding conditions, their inflexible body structures impede collision tolerance, necessitating operational spaces free of collisions. Recent years have witnessed an upsurge in integrating soft and pliable materials into the design of such systems; however, the pursuit of aerodynamic efficiency curtails the utilization of excessively flexible materials for rotor blades or propellers. This thesis introduces a design that integrates polyimide flexible PCBs into the wings of the Aerobat and employs guard design incorporating feedback-driven stabilizers, enabling stable hovering flights within Northeastern's Robotics-Inspired Study and Experimentation (RISE) cage.

==> Makefile <==
# ------------------------------------------------------------------------
# Makefile:
# ------------------------------------------------------------------------
# written by:	Gunar Schirner 
# External References:
#   http://kriemhild.uft.uni-bremen.de/viewvc/vim/Makefile.pdflatex
#   http://www.tex.ac.uk/tex-archive/help/uk-tex-faq/Makefile
# last update:	$id$
#
# Help screen (start every help line with #h)
#
#h make        builds ALL_REF
#h
#h make publish 
#h             publish the build output to HTML publish directory  
#h
# --- names --------------------------------------------------------------

PROJECT	=	thesis

SRCNAME	=	$(PROJECT)_SRC.tar.gz
BINNAME	=	$(PROJECT)_BIN.tar.gz
ORIG	=	

TMP	=	/tmp
# own name
MAKEF   =       Makefile

# path for automatic publishing, put into your public_html directory`
PUBLISH_PATH = /home/student/<studentName>/public_html/thesis
VERSION_FILE = svnRev.tex

# set automatically by hook script (Post commit hook)
# SVN_REPO_PATH 
# SVN_REV

# --- lists --------------------------------------------------------------

ALL	=	$(PROJECT).pdf



# auto use all *.tex file in the own and in pi directory as dependency input 
INCLUDE	:=	$(shell [ -d tex ] && echo tex/*.tex )

SOURCES =	$(PROJECT).tex	\
		$(INCLUDE)

#BIBFILES :=  macro/bib-strings.bib macro/IEEEabrv.bib $(shell [ -d bib ] && echo bib/*.bib )

FIGFILES =

PPTFILES =	

PRNFILES =

# auto use all *.eps files in the fig directory as a dependency input 
#  FIGURES directory may not exist
# uncomment once first eps is added 
EPSFILES :=	$(shell [ -d fig ] && echo fig/*.eps) 


# auto use all *.pdf files in the fig directory as a dependency input 
#  FIGURES directory may not exist
# uncomment once first pdf is added 
#PDFFIGS :=	$(shell [ -d fig ] && echo fig/*.pdf) 


FIGURES	=	$(EPSFILES:.eps=.pdf) $(PDFFIGS)

#MACROS	=	macro/macros.tex

OTHERS	=	Makefile	


ORIGS	=	$(SOURCES) $(MACROS) $(OTHERS)

SRCTAR	=	$(SOURCES) $(MACROS) $(OTHERS)	\
		$(FIGFILES) $(PPTFILES) $(PRNFILES) $(EPSFILES)

BINTAR	=	$(ALL)

# --- environment --------------------------------------------------------

TEXINPUTS =	TEXINPUTS=.:MACROS:

TEXENV	=	$(TEXINPUTS)

# --- commands -----------------------------------------------------------

FIGPS	=	fig2dev -L ps
PRN2EPS	=	PATH=bin:$$PATH prn2eps
LATEX	=	$(TEXENV) latex
PDFLATEX =      pdflatex --interaction nonstopmode
BIBTEX	=	bibtex
DVIPS	=	dvips -Z -D 600 -t letter -Ppdf
PS2PDF	=	ps2pdf
EPS2PDF	=	epstopdf
PSSEL	=	psselect
TAR	=	gtar cvzf
RM	=	rm -f
MV	=	mv -f
MAKEIDX	=	makeindex
GV	=	ghostview
ECHO	=	echo
GREP	=	grep
WC	=	wc
CD	=	cd
CAT	=	cat
XLESS	=	xless
SPELL	=	nspell -t
SORT	=	sort -f
MAKEIDX	=	makeindex
DISTILL =       GS_OPTIONS="-dAutoFilterColorImages=false \
                            -dColorImageFilter=/FlateEncode" ps2pdf14
THUMBPDF=       thumbpdf --modes=dvips

# parse string to cause rebuild of latex
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right|Table widths have changed. Rerun LaTeX.|Linenumber reference failed)"

# parse string to cause rebuild of bibtex
RERUNBIB = "No file.*\.bbl|Citation.*undefined"



# --- general rules ------------------------------------------------------

.SUFFIXES:
.SUFFIXES:	.fig .ps .prn .eps .tex .bbl .pdf

.fig.ps:
	$(FIGPS) $*.fig $*.ps

.prn.eps:
	$(PRN2EPS) $*.prn $*.eps

#GS added automatic conversion for eps files, epstopdf packages seems
# not installed on this linux installation
.eps.pdf:
	$(EPS2PDF) $*.eps

.tex.bbl:
	$(LATEX) $*.tex
	$(BIBTEX) $*

# run pdflatex once and bib + subsequent pdflatex conditionally
%.pdf: %.tex
	$(PDFLATEX) $<
	@egrep -c $(RERUNBIB) $*.log && (bibtex $*;$(PDFLATEX) $<); true
	@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	@egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true


# --- rules --------------------------------------------------------------

all:		$(ALL)

# automatically produce help message by grep for sepcial comment lines 
help:;	@sed -n -e 's/^#h//p'  < $(MAKEF) | sed -e 's/ALL_REF/$(ALL)/g'

# second phase of the publish requires to get the current SVN version 
ifdef SECOND_PHASE
SVN_REV := $(shell svn info | sed -n -e 's/.*Revision: //p')
endif

# debug rule to print current version 
echo_ver:
	@echo $(SVN_REV)

# paste the current version information into tex file so that it 
# can be included into build
create_version_file: 
	@echo "\\newcommand{\\svnRevRef}{$(SVN_REV)}" > $(VERSION_FILE)


# actual publishing action 
autobuild_publish_2nd: create_version_file
	make >  $(PUBLISH_PATH)/z_buildlog.r$(SVN_REV).log
	set -e ; for f in $(basename $(filter %.pdf, $(ALL))); do        \
		rm -f $(PUBLISH_PATH)/$$f.r*.pdf;                         \
		cp $$f.pdf $(PUBLISH_PATH)/$$f.r$(SVN_REV).pdf;   \
		rm -f $(PUBLISH_PATH)/$$f.pdf; \
		ln -s $(PUBLISH_PATH)/$$f.r$(SVN_REV).pdf $(PUBLISH_PATH)/$$f.pdf ;  \
	done

# if the revision is already passed in as a parameter, we do not 
# need to trieve it again 
ifneq ("$(SVN_REV)", "")
# clean update build and publish 
publish: clean svn_up autobuild_publish_2nd
else
# cleanup, svn update and kick off second phase
publish: 
	make clean
	svn up
	make autobuild_publish_2nd SECOND_PHASE=1
endif

# helper rule to call svn update 
svn_up: 
	svn up


clean:
	$(RM) $(ALL)
	$(RM) *.ps *.pdf
	$(RM) *.dvi
	$(RM) *.toc *.lot *.lof *.log *.aux
	$(RM) *.idx *.ind *.ilg
	$(RM) *.inx *.srt
	$(RM) *.blg *.bbl
	$(RM) *.out
	$(RM) *.BAK *.bak *~
	$(RM) macro/*.BAK macro/*.bak macro/*~
	$(RM) texput.log
	$(RM) $(ORIG)

tar:
	-$(MV) $(SRCNAME) $(SRCNAME).bak
	-$(MV) $(BINNAME) $(BINNAME).bak
	-$(TAR) $(SRCNAME) $(SRCTAR)
	-$(TAR) $(BINNAME) $(BINTAR)

spell:
	$(SPELL) $(SOURCES)

orig:	$(ORIG)

todo:	$(ORIG)
	-$(GREP) -n "\.\.\.\." `$(CAT) $(ORIG)` >$(TMP)/todo
	$(WC) -l $(TMP)/todo ; $(XLESS) $(TMP)/todo ; $(RM) $(TMP)/todo &

1:
	$(LATEX) $(PROJECT).tex
	$(DVIPS) $(PROJECT).dvi -o $(PROJECT).ps

2:
	$(LATEX) $(PROJECT).tex
	$(LATEX) $(PROJECT).tex
	$(DVIPS) $(PROJECT).dvi -o $(PROJECT).ps


# --- project rules ---

$(PROJECT).pdf:  $(PROJECT).tex $(MACROS) $(INCLUDE) $(FIGURES) $(BIBFILES) 


summary.pdf:	summary.tex

$(PROJECT).ps: $(PROJECT).pdf
	pdf2ps $<

Description.ps: $(PROJECT).ps
	$(PSSEL) 1-15 $(PROJECT).ps Description.ps

Description.pdf:	Description.ps
	$(DISTILL) Description.ps Description.pdf


References.ps: $(PROJECT).ps
	$(PSSEL) 16- $(PROJECT).ps References.ps

References.pdf:	References.ps
	$(DISTILL) References.ps References.pdf


# --- other rules ---

$(ORIG):	$(ORIGS)
	$(ECHO) >$(ORIG) $(ORIGS)



#h dbgPrint   VAR=<varName> print content of variable <varName>
dbgPrint:
	@echo "$(VAR)=$($(VAR))"
# --- EOF ----------------------------------------------------------------


==> bib/thesis.tex <==
% ----------------------------------------------------------------------------
% Citation database
% ----------------------------------------------------------------------------

@STRING{ASPDAC = "Proceedings of the Asia and South Pacific Design Automation Conference (ASPDAC)"}
@STRING{DAC = "Proceedings of the Design Automation Conference (DAC)"}
@STRING{DATE = "Proceedings of the Design, Automation and Test in Europe (DATE) Conference"}
@STRING{CODES = "Proceedings of the International Symposium on Hardware-Software Codesign (CODES)"}
@STRING{EDAC = "Proceedings of the European Design Automation Conference (Euro-DAC)"}
@STRING{EDTC = "Proceedings of the European Design and Test Conference"}
@STRING{ICCD = "Proceedings of the International Conference on Computer Design (ICCD)"}
@STRING{ICCAD = "Proceedings of the International Conference on Computer Aided Design (ICCAD)"}
@STRING{ISSS = "Proceedings of the International Symposium on System Synthesis"}
@STRING{SASIMI = "Proceedings of the Workshop of Synthesis and System Integration of Mixed Information Technologies"}
@STRING{ESC = "Proceedings of the Embedded System Conference (ESC)"}
@STRING{TCAD = "IEEE Transactions on Computer-Aided Design of Intergrated Circuits and Systems (TCAD)"}
@STRING{TCOMP = "IEEE Transactions on Computers"}
@STRING{TSP = "IEEE Transactions on Signal Processing"}
@STRING{TVLSI = "IEEE Transactions on VLSI Systems"}
@STRING{TPDS = "IEEE Transactions on Parallel and Distributed Systems"}
@STRING{D&T = "IEEE Design and Test of Computers"}
@STRING{JACM = "Journal of the ACM"}
@STRING{TODAES = "ACM Transactions on Design Automation of Electronic Systems"}
@STRING{Kluwer = "Kluwer Academic Publishers"}
@STRING{Prentice = "Prentice Hall"}

@STRING{ICS = "Information and Computer Science"}
@STRING{UCI = "University of California, Irvine"}
@STRING{CECS = "Center for Embedded Computer Systems"}




% --- Books ---

% Applications

% Design languages and methodologies

@BOOK{book:SpecC:yellow,
   AUTHOR = "Andreas Gerstlauer and Rainer D{\"o}mer and Junyu Peng and
             Daniel D. Gajski",
   TITLE = "System Design: A Practical Guide with {SpecC}",
   PUBLISHER = Kluwer,
   YEAR = {2001}
}

@BOOK{book:SpecC:green,
   AUTHOR = "Daniel D. Gajski and Jianwen Zhu and Rainer D{\"o}mer and
             Andreas Gerstlauer and Shuqing Zhao",
   TITLE = "{SpecC}: Specification Language and Design Methodology",
   PUBLISHER = Kluwer,
   YEAR = {2000}
}

@BOOK{book:SystemC,
   AUTHOR = "Thorsten Gr{\"o}tker and Stan Liao and Grant Martin and Stuart Swan",
   TITLE = "System Design with {SystemC}",
   PUBLISHER = Kluwer,
   YEAR = {2002}
}


% Design environments

@BOOK{book:SpecSyn,
    AUTHOR = "Daniel D. Gajski and Frank Vahid and Sanjiv Narayan and Ji Gong",
    TITLE = "Specification and Design of Embedded Systems",
    PUBLISHER = Prentice,
    YEAR = {1994}
}

@BOOK{book:polis,
    AUTHOR = "Felice Balarin and Massimiliano Chiodo and Paolo Giusto and
              Harry Hsieh and Attila Jurecska and Luciano Lavagno and
              Claudio Passerone and Alberto Sangiovanni-Vincentelli and
              Ellen Sentovich and Kei Suzuki and Bassam Tabbara",
    TITLE = "Hardware-Software Co-Design of Embedded Systems: 
             The {POLIS} Approach",
    PUBLISHER = Kluwer,
    YEAR = {1997}
}



% --- Journal papers ---

% Design languages

% papers

@INPROCEEDINGS{paper:lang:SpecC:formal,
   AUTHOR = "Wolfgang Mueller and Rainer D{\"o}mer and Andreas Gerstlauer",
   TITLE  = "The Formal Execution Semantics of {SpecC}",
   BOOKTITLE = ISSS,
   ADDRESS = {Kyoto, Japan},
   MONTH = {October},
   YEAR = {2002}
}

@INPROCEEDINGS{paper:lang:SpecC,
   AUTHOR = "Jianwen Zhu and Rainer D{\"o}mer and Daniel D. Gajski",
   TITLE  = "Syntax and Semantics of the {SpecC} Language",
   BOOKTITLE = ISSS,
   ADDRESS = {Osaka, Japan},
   MONTH = {December},
   YEAR = {1997}
}

@MISC{latex:index,
	AUTHOR = "Wikibooks",
	TITLE  = "LaTeX/Indexing",
	HOWPUBLISHED = {\url{http://en.wikibooks.org/wiki/LaTeX/Indexing}}
}


%%% most important :-) 
@book {book:42,
	author = "Douglas Adams",
	title = "The Hitchhiker's Guide to the Galaxy",
	publisher = "Pan Books",
	year = 1979,
	month = oct,
}
